A Deep Learning Approach to the Inversion of Borehole Resistivity Measurements

We use borehole resistivity measurements to map the electrical properties of the subsurface and to increase the productivity of a reservoir. When used for geosteering purposes, it becomes essential to invert them in real time. In this work, we explore the possibility of using Deep Neural Network (DNN) to perform a rapid inversion of borehole resistivity measurements. Herein, we build a DNN that approximates the following inverse problem: given a set of borehole resistivity measurements, the DNN is designed to deliver a physically meaningful and data-consistent piecewise one-dimensional layered model of the surrounding subsurface. Once the DNN is built, we can perform the actual inversion of the field measurements in real time. We illustrate the performance of DNN of logging-while-drilling measurements acquired on high-angle wells via synthetic data.

==> Figures/data_area.tex <==
\begin{tikzpicture}

\draw[fill,brown!40!white] (0,0) -- (6,0) -- (6,4) -- (0,4) -- (0,0);

\draw[fill,blue!40!white,rounded corners=1mm] (1.5,2) \irregularcircle{1cm}{1mm};
\draw[thick,<-] (2.6,2.1) -- (3.1,3.) node[anchor=south] {Physical problems};
\node[align=left] at (2.1,0.3) {Unphysical problems};


\end{tikzpicture}

==> Model_1/1D.tex <==
%\tdplotsetmaincoords{60}{125}
\begin{tikzpicture}
\draw[fill=black!60!white] (0,0) -- (6,0) -- (6,1) -- (0,1) -- (0,0);
\node (z5) at (3,0.5) {$\rho_4$};
\node (z1) at (-0.5,4) {0};
\draw[fill=gray!70!white] (0,1) -- (6,1) -- (6,2) -- (0,2) -- (0,1);
\node (z5) at (3,1.5) {$\rho_3$};
\node (z2) at (-0.5,3) {7.5};
\draw[fill=brown!70!white] (0,2) -- (6,2) -- (6,3) -- (0,3) -- (0,2);
\node (z5) at (3,2.5) {$\rho_2$};
\node (z3) at (-0.5,2) {15};
\draw[fill=brown!30!white] (0,3) -- (6,3) -- (6,4) -- (0,4) -- (0,3);
\node (z5) at (3,3.5) {$\rho_1$};
\node (z4) at (-0.5,1) {22.5};
\node (z5) at (-0.5,0) {30};
\node[rotate=90] (z5) at (-1.5,2) {True vertical depth};
\draw[thick, magenta] (0,4) -- (6,0) node (n1) at (0.5,3.4) {T};
\end{tikzpicture}

==> Model_1/Fig_tool1.tex <==
\begin{tikzpicture}

%% Tool
\fill[gray!80!white] (-1.5*3,0) -- (1.5*3,0.) --  node[right] {\small \bf \textcolor{black}{1 MHz}}  (1.5*3, 0.15*3) -- (-1.5*3,0.15*3) -- cycle;

%% Transmitters
\fill[black!80!white] (-0.6096*5-0.02*3,0) -- (-0.6096*5+0.02*3,0.) -- (-0.6096*5+0.02*3, 0.15*3) node[above] {\footnotesize \bf \textcolor{black}{Tx$_1$}}  -- (-0.6096*5-0.02*3,0.15*3) -- cycle;
%
\fill[black!80!white] (0.6096*5-0.02*3,0) -- (0.6096*5+0.02*3,0.)  -- (0.6096*5+0.02*3, 0.15*3) node[above] {\footnotesize \bf \textcolor{black}{Tx$_2$}} -- (0.6096*5-0.02*3,0.15*3) -- cycle;

%% Receivers
\fill[red!80!white] (-0.1016*5-0.02*3,0) -- (-0.1016*5+0.02*3,0.)  -- (-0.1016*5+0.02*3, 0.15*3) node[above] {\footnotesize \bf \textcolor{black}{Rx$_1$}} -- (-0.1016*5-0.02*3,0.15*3) -- cycle;
\fill[red!80!white] ( 0.1016*5-0.02*3,0) -- ( 0.1016*5+0.02*3,0.) -- ( 0.1016*5+0.02*3, 0.15*3)  node[above] {\footnotesize \bf \textcolor{black}{Rx$_2$}} -- ( 0.1016*5-0.02*3,0.15*3) -- cycle;

%% distances
\draw[black, line width=1pt,<->] (-0.1016*5, -0.6)      -- (0.1016*5, -0.6) node[pos=0.5, below] {\footnotesize \bf \textcolor{black}{0.40 m}}  ;
\draw[gray, dashed] (-0.1016*5, -0.6)      -- (-0.1016*5, 0)  ;
\draw[gray, dashed] ( 0.1016*5, -0.6)      -- ( 0.1016*5, 0)  ;

\draw[black, line width=1pt,<->] (-0.6096*5, -1.2)      -- (0.6096*5, -1.2) node[pos=0.5, below] {\footnotesize \bf \textcolor{black}{2 m}}  ;
\draw[gray, dashed] (-0.6096*5,-1.2)      -- (-0.6096*5, 0)  ;
\draw[gray, dashed] ( 0.6096*5,-1.2)      -- ( 0.6096*5, 0)  ;


\end{tikzpicture}

==> adrian.tex <==
\section{Deep Neural Networks for Inverting Resistivity Measurements}
\label{sec:deep_learning}
In this section, we consider a discrete representation of the inverse function ${\bf I}_h:\boldsymbol{\cal M}\times {\bf T} \rightarrow {\bf P}$ that associates each pair of measurements and trajectories $(m, t)\in \boldsymbol{\cal M}\times {\bf T}$ with a corresponding distribution of subsurface properties $P \in {\bf P}$. In order to approximate this function, we employ Neural Networks (NNs) \cite{hornik_approximation_1991}. We provide below a concise overview of how to construct this kind of operators. The existing literature about NNs is large, but in here we only intend to briefly introduce geophysicists on some NNs and related algorithms that seem to be relevant for the inversion of borehole resistivity measurements.

\subsection{Fully-Connected Neural Network Definition}\label{nn}
%Let us consider a NN ${\bf I}_\theta$ defined by $\theta$, which denotes a large vector of free parameters.
Early formulations of NNs, known as Fully-Connected Neural Networks (FC-NNs), were defined by repeated compositions of simple transformations. Denoting $x=(m, t)$, a FC-NN composed of $L$ \textit{layers} is given by:
\begin{equation}\label{nn_eq}
{\bf I}_\theta(x) = (\mathcal{N}^{(L)} \circ \ldots \circ \mathcal{N}^{(l)}\circ \ldots \mathcal{N}^{(2)} \circ \mathcal{N}^{(1)})(x),
\end{equation}
where $\mathcal{N}^{(l)}(x) = \mathbf{s}(W^{(l)} \cdot x + b^{(l)})$ , $W^{(l)}$ is a matrix, and $b^{(l)}$ a vector. Thus, $W^{(l)} \cdot x + b^{(l)}$ is an affine transformation. ${\bf s}$ is a simple non-linear point-wise mapping, typically the so-called \textit{half-sided rectifier} given by:
%is an affine transformation of an input $x$ followed by a non-linear point-wise mapping, typically a half-sided rectifier given by:
\begin{equation}\label{activation}
\mathbf{s}({v_1,...,v_r})=(\max(0,v_1),...,\max(0,v_r)).
\end{equation}
We define $\theta^{(l)}$ as a vector composed of all entries of matrices $W^{(l)}$ and vectors $b^{(l)}$ for each layer $l=1,...,L$. Thus, $\theta = \{\theta^{(l)} \ : \ 1\leq l \leq L\}$ is a large vector of parameters fully determining ${\bf I}_\theta$. 
Due to the varying dimensions of the different matrices $W^{(l)}$, and vectors $b^{(l)}$ at each layer in Equation \eqref{nn_eq}, the dimensionality of the input $x$ can change, so it eventually reaches that of the target variable ${P \in\bf P}$.

% where $\mathcal{A}^{(l)}(x) = W^{(l)} \cdot x + b^{(l)}$ is an affine transformation of its input $x$. To let the network approximate more complex non-linear operators, each of these transformations is followed by a non-linear point-wise mapping, typically a half-sided rectifier $s(z)=\max(0,z)$. We define $\theta^{(l)}$ as a vector composed of all entries of matrices $W^{(l)}$ and vectors $b^{(l)}$ for each layer $l=1,...,L$, in such a way that $\theta = \{\theta^{(l)} \ : \ 1\leq l \leq L\}$ is a large vector of parameters that fully defines ${\bf I}_\theta$.



\subsection{Training a Neural Network: Data Preparation}
We consider a finite set $S$ containing $m$ data samples:
\begin{equation}\label{global_set}
S=(M, T, P) = \{(m^{[i]}, t^{[i]}, \rho^{[i]}) \ : \  m^{[i]} \in \boldsymbol{\cal M}, t^{[i]} \in {\bf T}, P^{[i]}\in {\bf P}, \ 1\leq i \leq m\}.
\end{equation}
This set is randomly split into three disjoint subsets, referred to as \textit{training}, \textit{validation}, and \textit{test} sets, respectively:
\begin{align}
S_{train} &= (M_{\mathrm{train}},T_{\mathrm{train}},P_{\mathrm{train}}) = \{(m^{[i]}, t^{[i]}, P^{[i]}) \ : \ 1\leq i \leq m_1\},\\
S_{val} &= (M_{\mathrm{val}},T_{\mathrm{val}},P_{\mathrm{val}}) = \{(m^{[i]}, t^{[i]}, P^{[i]}) \ : \ m_1+1\leq i \leq m_2\},\\
S_{test} &= (M_{\mathrm{test}},T_{\mathrm{test}},P_{\mathrm{test}}) = \{(m^{[i]}, t^{[i]}, P^{[i]}) \ : \ m_2+1\leq i \leq m\}.
\end{align}
We apply a network ${\bf I}_\theta$ to input data sampled from set $S$ in order to produce a prediction ${\bf I}_\theta(m^{[i]}, t^{[i]})$ of its resistivities. Then, one can compute the accuracy of such prediction via an error function $\mathcal{L}$, e.g., the $\mathit{l}_2$ norm of the difference between both vectors:
\begin{equation}\label{loss}
\mathcal{L}({\bf I}_\theta(m^{[i]}, t^{[i]}), P^{[i]}) = \|{\bf I}_\theta(m^{[i]}, t^{[i]})-P^{[i]}\|_{2}
\end{equation}
The numerical process by which the error given by Equation \eqref{loss} is iteratively minimized via a gradient-based algorithm across the entire training set is referred to as \textit{training}, and will be detailed in the next subsection. The validation set $S_{val}$ is employed to perform some high-level NN design decisions, e.g., to modify the network architecture (the dimensions of the different layers) or different parameters controlling the numerical optimization algorithm. After training, we compute predictions for data samples in $S_{test}$ . Then, the network ${\bf I}_\theta$ is generalize properly if the errors in $S_{train}$ and $S_{test}$ are similar. In addition, if such errors are relatively low, we can assume that ${\bf I}_\theta$ correctly approximates operator $\mathbf{I}_h$.


\subsection{Training a Neural Network: Numerical Optimization}
%In order to minimize the error $\mathcal{L}$ of eq. (\ref{loss}) over the training set $S_{train}$, standard approaches include first-order gradient-based schemes. 
A critical feature of NN is that they are a hierarchical composition of multiple functions which are easy to differentiate. Hence, the chain rule becomes an essential tool to find derivatives of these operators. This is the core idea of the most popular algorithm for implementing gradient descent strategies on NNs, called \textit{back-propagation} in the NN's literature \cite{rumelhart_parallel_1986}.

Within each gradient descent iteration, we first carry out a forward pass for a given data sample $(m_i, t_i)$ in order to compute a prediction ${\bf I}_\theta(m_i, t_i)$ and the corresponding error $\mathcal{L}({\bf I}_\theta(m_i, t_i),P_i)$. Afterwards, this error is backpropagated by applying the chain rule to the composition of functions defining the different layers of the network. Hence, proceeding from the last layer of the model backwards, one can compute the gradient estimates of the loss function with respect to parameters $\theta$ defining ${\bf I}_\theta$ in reverse order as:
\begin{equation} 
\frac{\displaystyle \partial \mathcal{L}(\theta)}{\displaystyle \partial \theta^{(L)}}, 
\ldots, 
\frac{\displaystyle \partial \mathcal{L}(\theta)}{\displaystyle \partial \theta^{(l+1)}},
\frac{\displaystyle \partial \mathcal{L}(\theta)}{\displaystyle \partial \theta^{(l)}},
\ldots,
\frac{\displaystyle \partial \mathcal{L}(\theta)}{\displaystyle \partial\theta^{(1)}}
\end{equation}
The gradient at each layer is derived based on previous gradient computations, parameters $\theta$ are updated with some form of gradient descent strategy (e.g., stochastic gradient descent), and the process is iterated over all elements of the training set so as to minimize its error. 

The number of iterations during which the model is trained is typically decided by monitoring the value of the loss function $\mathcal{L}$ on elements of the validation set $S_{val}$ that are never used to adjust the network parameters. 
During training, that value is compared with the loss value attained in $S_{train}$ in order to stop the optimization process as soon as both quantities start to diverge, which would imply that the network is becoming {\em too} much adjusted to the training data and failing to generalize, a phenomenon known as \textit{overfitting}.

\subsection{Convolutional Neural Networks}
As observed from Equation \eqref{nn_eq}, NNs are defined as a composition of functions. Thus, they naturally possess a layer-wise hierarchical nature. Therefore, they are ideal candidates to design operators that progressively retain the most salient aspects of the initial input. However, $W^{(l)}$ are dense matrices, connecting every component of the input of a given layer to its output. This results in an excessively large number of parameters that need to be optimized. In order to reduce this number, a popular solution consists of replacing fully-connected affine layers $\mathcal{N}$ by convolutional operators $\mathcal{C}$ defined by convolution kernels $f$. This localizes computations, effectively reducing the number of parameters in ${\bf I}_\theta$. The resulting network is known as a Convolutional Neural Network (CNN) \cite{lecun_gradient-based_1998}. We provide a rigorous definition of a CNN in Appendix \ref{convolutional}.

\subsection{Recurrent Neural Networks}
A particular kind of network architectures that are useful for sequence processing (\textit{e.g.} speech, text, or time-related data) are Recurrent Neural Networks (RNNs) \cite{hopfield_neural_1982}. In here, since successively recorded logging data exhibit a temporal pattern (there is a strong relationship between measurements recorded at a given logging position and the next one), we also adopt a RNN. For a technical description of this type of networks, see Appendix \ref{recurrent}.


\subsection{A Neural Network Architecture for Inverting Borehole Resistivity Measurements}
The NN architecture employed in this work combines both a CNN and a RNN by first reducing the dimensionality of the input measurements employing a Long Short-Term Memory Network, a specific class of RNN described in Appendix \ref{recurrent}. Next, the result of this operation serves as input to a series of one-dimensional CNN, with interleaved \textit{pooling} operators similar to the ones described in Appendix \ref{convolutional}, where each convolutional block is based on a modified residual block \cite{He}, allowing deeper architectures while enhancing convergence. The output of this second set of operations becomes the input to a fully-connected layer that maps it into space ${\bf P}$ of subsurface resistivity properties. The network is trained end-to-end by backpropagation until the validation error is no longer decreasing. We provide A pseudo-code of this DNN in Appendix \ref{code}.




